Goldstone Equivalence and High Energy Electroweak Physics

The transition between the broken and unbroken phases of massive gauge theories, namely the rearrangement of longitudinal and Goldstone degrees of freedom that occurs at high energy, is not manifestly smooth in the standard formalism. The lack of smoothness concretely shows up as an anomalous growth with energy of the longitudinal polarization vectors, as they emerge in Feynman rules both for real on-shell external particles and for virtual particles from the decomposition of the gauge field propagator. This makes the characterization of Feynman amplitudes in the high-energy limit quite cumbersome, which in turn poses peculiar challenges in the study of Electroweak processes at energies much above the Electroweak scale. We develop a Lorentz-covariant formalism where polarization vectors are well-behaved and, consequently, energy power-counting is manifest at the level of individual Feynman diagrams. This allows us to prove the validity of the Effective W Approximation and, more generally, the factorization of collinear emissions and to compute the corresponding splitting functions at the tree-level order. Our formalism applies at all orders in perturbation theory, for arbitrary gauge groups and generic linear gauge-fixing functionals. It can be used to simplify Standard Model loop calculations by performing the high-energy expansion directly on the Feynman diagrams. This is illustrated by computing the radiative corrections to the decay of the top quark.

==> Applications/app_splittings.tex <==


The splitting density matrix $d\rho^{\rm{split}}$, differential in the variables $\phi$, $|{\bf{k_\bot}}|$ and $x$ that characterise the splitting is the generalization, to include interference effects, of the ordinary splitting functions. \Gabriel{Di solito si definisce $\rho=\mathcal{M}^*\mathcal{M}$, vedi eq. 1.106 \href{http://scipp.ucsc.edu/~haber/webpage/ssi93.pdf}{qui}. \href{https://arxiv.org/pdf/1611.00788.pdf}{Tao Han} (app. C) usa invece $dP$ come facciamo sotto. In base a quello che scriviamo per initial state radiation:}
\begin{eqnarray}
d\rho^{\rm{split}}_{C_h\,C_{h'}'} &=&\frac{x(1-x)}{16\pi^2} \frac{\M^{\rm split}(A\rightarrow BC_{h})[\M^{\rm split}(A\rightarrow BC_{h'}')]^*}{{\widetilde k}_\bot^2(m_A,m_B,m_C)~~{\widetilde k}_{\bot}^2(m_{A},m_{B},m_{C'})}dx\,d|{\bf k}_\bot|^2d\phi\,,\\
d\rho^{\rm{hard}}_{C_h\,C_{h'}'}&=&\frac{\M^{\rm hard}(C_hX\rightarrow Y)[\M^{\rm hard}(C_{h'}'X\rightarrow Y)]^*}{4E_XE_C|{\bf v}_C-{\bf v}_X|}(2\pi)^4\delta^{(4)}(k_Y-k_C-k_X)d\Phi_Y\,.
\end{eqnarray}
\Gabriel{Per final state radiation:}
\begin{eqnarray}
d\rho^{\rm{split}}_{A_h\,A_{h'}'} &=&\frac{x(1-x)}{16\pi^2} 
\frac{\M^{\rm split}(A_h\rightarrow BC)[\M^{\rm split}(A_{h'}'\rightarrow BC)]^*}{{\widetilde k}_\bot^2(m_A,m_B,m_C)~~{\widetilde k}_{\bot}^2(m_{A'},m_{B},m_{C})}dx\,d|{\bf k}_\bot|^2d\phi\,,\\
d\rho^{\rm{hard}}_{A_h\,A_{h'}'}&=&\frac{\M^{\rm hard}(X\rightarrow A_hY)[\M^{\rm hard}(X\rightarrow A_{h'}' Y)]^*}{4E_{X_1}E_{X_2}|{\bf v}_{X_1}-{\bf v}_{X_2}|}(2\pi)^4\delta^{(4)}(k_Y+k_A-k_X)d\Phi_Y d\Phi_A\,.\qquad
\end{eqnarray}
\Gabriel{Lo spazio delle fasi su B e Y \`e (a meno della $(2\pi)^4\delta^{(4)}(\ldots)$)}
\begin{equation}
d\Phi=d\Phi_B d\Phi_Y=
\frac{d^3k_B}{2E_{B}(2\pi)^3}\prod_{f\in Y}\frac{d^3 k_f}{2E_f(2\pi)^3}=
\frac{dx\,d|{\bf k}_\bot|^2\,d\phi}{4(1-x)(2\pi)^3}
\left[1+\mO\left(\delta_\bot^2\right)\right]\prod_{f\in Y}\frac{d^3 k_f}{2E_f(2\pi)^3}\,.
\end{equation}
\Gabriel{Forse in modo pi\`u compatto si pu\`o scrivere per i $d\rho$:}
\begin{eqnarray}
d\rho^{\rm{split}}_{A\to B C; A'\to B' C'} &=&\frac{x(1-x)}{16\pi^2} \frac{\M^{\rm split}(A\rightarrow BC)[\M^{\rm split}(A'\rightarrow B'C')]^*}{{\widetilde k}_\bot^2(m_A,m_B,m_C)~~{\widetilde k}_{\bot}^2(m_{A'},m_{B'},m_{C'})}dx\,d|{\bf k}_\bot|^2d\phi\,,\\
d\rho^{\rm{hard}}_{X\to Y; X'\to Y'}&=&\frac{\M^{\rm hard}(X\rightarrow Y)[\M^{\rm hard}(X'\rightarrow Y')]^*}{4E_{X_1}E_{X_2}|{\bf v}_{X_1}-{\bf v}_{X_2}|}(2\pi)^4\delta^{(4)}(k_Y-k_X)d\Phi_Y\,.
\end{eqnarray}

with . Eq. \eqref{virtuality} of course holds up to ${\cal O}(\delta_{\bot, m}^2)$ corrections.


We next move to the differential cross sections for the two processes in Fig \ref{fig_fact}. In addition to the different virtualities in \eqref{virtuality}, another important difference between the two reactions is found in the phase space. We begin with the process $AX\to BY$, and assume $X$ is a single particle state, as it turns out to be in all practical situations. We then compute the differential cross section in the final state phase space $d\Phi_Y$ as well as the energy and transverse momentum of the emitted $B$. This is derived integrating solely over the azimuthal angle $\phi$ defined in \eqref{eq:kin}. The final state phase space contains a factor $d{\vec k}_{B}/[2E_{B}(2\pi)^3]=d|{\bf k}_\bot|^2\,dx\,d\phi/[4(1-x)(2\pi)^3][1+{\cal O}(|{\bf k}_\bot|^2/k_z^2)]$ from the forward $B$, times of course $d\Phi_Y=\prod_{f\in Y}d{\vec k}_f/[2E_f(2\pi)^3]$ with $f$ denoting any of the one-particle states contained in $Y$. Observing that, at leading order in $\delta_{m,\bot}$, the azimuthal angle $\phi$ appears only in the splitting functions, and using angular momentum conservation, namely $\int d\phi~\M^{\rm split}(A\rightarrow BC_h)\left[\M^{\rm split}(A\rightarrow BC_{h'})\right]^*=2\pi\left|\M^{\rm split}(A\rightarrow BC_h)\right|^2\delta_{h h'}$, we obtain
%\ba\label{XS:in}
%d\sigma_{A X\rightarrow B Y}&=&\sum_{h}
%\frac{d^2{P}_{A\rightarrow BC_h}}{dx\,d|{\bf k}_\bot|^2}dx\,d|{\bf k}|^2_\bot
%\times \frac{d\sigma_{C_h X\rightarrow Y}}{d\Phi_Y}d\Phi_Y\times[1+{\cal O}(\delta^2)]\\\no
%\frac{d^2{P}_{A\rightarrow BC_h}}{dx\,d|{\bf k}_\bot|^2}&=&
%\frac{x}{16\pi^2(1-x)}
%\frac{|\M^{\rm split}(A\rightarrow BC)|^2}{V^4}\\\no
%&=& \frac{x(1-x)}{16\pi^2}
%\frac{|\M^{\rm split}(A\rightarrow BC)|^2}{\widetilde k_\bot^4}.
%\ea
%\ba\no
%\frac{d\sigma_{A X\rightarrow B Y}}{d\Phi_Y}&=&\sum_{h}\sum_{C,C'}\frac{\M^{\rm hard}(C_hX\rightarrow Y)[\M^{\rm hard}(C_h'X\rightarrow Y)]^*}{4E_XE_C|1-v_X|}(2\pi)^4\delta^{(4)}(k_Y-k_C-k_X)\\\label{XS:in}
%&\times&dx\,d|{\bf k}_\bot|^2\frac{x(1-x)}{16\pi^2} \frac{\M^{\rm split}(A\rightarrow BC_h)[\M^{\rm split}(A\rightarrow BC_h')]^*}{{\widetilde k}_\bot^2(m_A,m_B,m_C)~~{\widetilde k}_{\bot}^2(m_A,m_B,m_{C'})}\times[1+{\cal O}(\delta^2)]\,,
%\ea
\ba\no
\frac{d\sigma_{A X\rightarrow B Y}}{d\Phi_Ydx\,d|{\bf k}_\bot|^2}&=&\sum_{h}\sum_{C,C'}\frac{\M^{\rm hard}(C_hX\rightarrow Y)[\M^{\rm hard}(C_h'X\rightarrow Y)]^*}{4E_XE_C|{\bf v}_C-{\bf v}_X|}(2\pi)^4\delta^{(4)}(k_Y-k_C-k_X)
\\\label{XS:in}
&\times&\frac{dP_{A\to B C_h; A\to B C_h'}}{dx\,d|{\bf k}_\bot|^2}\times[1+{\cal O}(\delta^2)]
\ea
where we introduced the differential splitting ``probability"
\ba\label{dPsplit}
\frac{dP_{A\to B C; A'\to B' C'}}{dx\,d|{\bf k}_\bot|^2}=\frac{x(1-x)}{16\pi^2} \frac{\M^{\rm split}(A\rightarrow BC)[\M^{\rm split}(A'\rightarrow B'C')]^*}{{\widetilde k}_\bot^2(m_A,m_B,m_C)~~{\widetilde k}_{\bot}^2(m_{A'},m_{B'},m_{C'})}\,.
\ea
In eq. \eqref{XS:in} we also used $E_A= E_C/x[1+{\cal O}(\delta_m^2)]$, from which one factor of $x$ arises in the numerator of \eqref{dPsplit}. Also, the hard amplitudes $\M^{\rm hard}(C_hX\rightarrow Y)$ are calculated with a collinear $C$ momentum 
\ba\label{kCcoll}
k^\mu_{C, \rm coll}=(\sqrt{x^2 k_z^2+m_C^2},0,0,x k_z)\,,
\ea
{\color{red}clarify}. Note we included also the effect of possible interferences among diagrams with different species of $C$, as indicated in eq. \eqref{fact}. It is understood that at the order of interest $k_C^\mu=k_{C'}^\mu[1+{\cal O}(\delta_m^2)]$ and $E_C\approx E_{C'}\approx xE_A$. In the absence of interference the first line of \eqref{XS:in} simply reduces to the differential cross section $\sum d\sigma_{C_hX\rightarrow BY}/{d\Phi_Y}$ and $\int dP$ can be interpreted as a splitting probability.














Remarkably, all corrections to the factorized cross-section are ${\cal O}(\delta^2)$. This is quite non-trivial because factorization of the amplitude was shown to hold up to ${\cal O}(\delta)$, see \eqref{fact}. %Yet, after having taken the square and integrated over $\phi$, the latter uncertainty translates into a much smaller ${\cal O}(\delta^2)$ effect in the relevant regime \eqref{condFacto}. 
This somewhat unexpected improvement in the accuracy was pointed out in the context of the Effective W approximation by the authors of \cite{EWA_Wulzer}. {\color{red}clarify} Their argument exploits the spurious symmetry \eqref{spuriousS} and the consequent fact that the hard matrix element for longitudinal and transverse vectors have a different scaling with energy. We shall not repeat that consideration here, but simply observe that the very same logic can be followed without changes in the GE formalism, and applies to arbitrary processes.












A similar procedure gives a factorized expression for the cross section of a process $X\rightarrow YBC$, with $X=X_1+X_2$, where the splitting is in the final state. In the limit $-Q^2=(k_B+k_C)^2\ll E^2$ we get
%\ba\label{XS:fin}
%d\sigma_{X\rightarrow YBC}&=&\sum_{h}
%\frac{d^2\sigma_{X\rightarrow YA_h}}{d\Phi_Yd\Phi_A}d\Phi_Yd\Phi_A\times \frac{d^2{P}_{A_h\rightarrow BC}}{dx\,d|{\bf k}_\bot|^2}dx\,d|{\bf k}|^2_\bot
%\times [1+{\cal O}(\delta^2)]\\\no
%\frac{d^2{P}_{A_h\rightarrow BC}}{dx\,d|{\bf k}_\bot|^2}&=&
%\frac{1}{16\pi^2x(1-x)}
%\frac{|\M^{\rm split}(A\rightarrow BC)|^2}{V^4}\\\no
%&=&
% \frac{x(1-x)}{16\pi^2}
%\frac{|\M^{\rm split}(A\rightarrow BC)|^2}{\widetilde k_\bot^4},
%\ea
\ba\no
\frac{d\sigma_{X\rightarrow BC Y}}{d\Phi_Ydx\,d|{\bf k}_\bot|^2}&=&\sum_{h}\sum_{A,A'}d\Phi_A\frac{\M^{\rm hard}(X\rightarrow A_hY)[\M^{\rm hard}(X\rightarrow A_h'Y)]^*}{4E_{X_1}E_{X_2}|{\bf v}_{X_1}-{\bf v}_{X_2}|}(2\pi)^4\delta^{(4)}(k_Y+k_A-k_X)\\\label{XS:fin}
&\times&\frac{dP_{A_h\to B C; A'_h\to B C}}{dx\,d|{\bf k}_\bot|^2}\times[1+{\cal O}(\delta^2)],
\ea
with $d\Phi_A=d{\vec k}_A/2E_A(2\pi)^3$ and ${\vec k}_A$ parametrized in \eqref{eq:kin_gen}. Similarly to \eqref{XS:in}, in the absence of interference among the virtual $A,A'$ states the first line of \eqref{XS:fin} becomes $\sum d\sigma_{X\rightarrow A_hY}/{d\Phi_Y}$. As explained above, eq. \eqref{XS:fin} holds up to corrections of order $\delta_{m,\bot}^2$.
%, as opposed to what we found for example in \eqref{eq-EWA_proof} for the helicity amplitudes of a unique species $C$. 


We stress that the differential splitting ``probability" in the second line in \eqref{XS:fin} is completely analogous to that in \eqref{XS:in}, and the two exactly coincide in the absence of interference among different species, despite the fact that the virtualities in the two processes are different. 












\section{Conclusions}\label{sec:conclusions}


\Gabriel{ho copiato qua alcuni commenti che avevo messo in EWA}
Finally, let us comment on the inclusion of loop effects. As argued in \Gabriel{metti}, a decomposition of the propagator similar to \eqref{Mres} holds at any order in perturbation theory. Then following the same steps one might be tempted to conclude that the proof of EWA proceeds in the same way, but for a proper inclusion of some form factors in the definition of splitting amplitudes. This reasoning however does not take into account infrared singularities which arise through soft and collinear loop effects, which must be properly resummed and complicate the proof. We leave an investigation of this issue for future work.//
Many works in the last years studied the properties of infrared singularities in the $m_W\rightarrow 0$ limit of the SM, showing that these might lead to physical suppression for sufficiently inclusive cross sections at high energy \cite{}. We hope the Goldstone Equivalent approach, allowing to correctly keep track of symmetry breaking effects, will allow to make further progress in the study of soft and collinear radiation in the SM at high energy.

\section*{Acknowledgements}

G.C. acknowledges A.Hebbar, K.Mimouni, L.Ricci and R.Rattazzi for useful discussions. The work of G.C. is partially supported by the Swiss National Science Foundation under contract 200020-169696 and through the National Center of Competence in Research SwissMAP. 



\appendix





%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Splitting in the Standard Model}\label{app-splitting}
\label{app:split}
%%%%%%%%%%%%%%%%%%%%%%%%%


In this appendix we derive explicit expressions for the splitting amplitudes \eqref{splitGen}. These depend on the definition of single particle states, which themselves determine the form of the polarization vectors (up to a conventional phase). We hence first present the conventions used throughout the paper. Then we discuss a few key properties of the splitting amplitudes and derive the identities \eqref{BCCB} and \eqref{CPsplit} that may be used by the reader to calculate the splitting amplitudes we do not quote explicitly. Finally, we list all splitting amplitudes relevant for Standard Model processes. 


 

\subsection{Preliminaries}

\subsubsection*{Conventions for 1-Particle States and Polarization Vectors} 

We define particles in the helicity basis following ref. \cite{Jacob:1959at}. 1-particle states of mass $m$, helicity $h$, and 3-momentum 
\ba\label{3momentum}
{\vec k}=\left(k_x, k_y, k_y\right)
=|{\vec k}|\left(
\sin\Theta\cos\Phi,
\sin\Theta\sin\Phi,
\cos\Theta
\right)
\ea
are obtained acting on a reference state $|{\vec k}_{\rm ref},h\rangle$ (to be specified below) with the standard Lorentz transformation $\Lambda_{\vec k}=R_{\rm JW}(\Theta,\Phi)\,e^{+i\eta K_3}$
\begin{equation}\label{eq:DefHelicity}
|{\vec k},h\rangle\equiv U(\Lambda_{\vec k})|{\vec k}_{\rm ref},h\rangle\,,
\end{equation} 
where  $R_{\rm JW}(\Theta,\Phi)$ is defined in \eqref{eq:R_jacob_wick}, and $K_3$ is the generator of boosts along the $z$ axis. The reference state $|{\vec k}_{\rm ref},h\rangle$ and the value of the rapidity $\eta$ in \eqref{eq:DefHelicity} depend on whether the associated particle is massless or massive. If $m=0$ the reference state has 3-momentum ${\vec k}_{\rm ref}=+|{\vec k}_{\rm ref}|{\vec z}$ along the positive $z$ direction and helicity $h={\vec k}_{\rm ref}\cdot{\vec J}/|{\vec k}_{\rm ref}|$. By definition $\Lambda_{\vec k}$ is such that $k^\mu=[\Lambda_{\vec k}{k}_{\rm ref}]^\mu$ and requires $\ln\eta=|{\vec k}|/|{\vec k}_{\rm ref}|$. When $m\neq0$ the reference state $|{\vec k}_{\rm ref},h\rangle$ has vanishing 3-momentum, $k_{\rm ref}^\mu=(m, {\vec 0})$, and its $h=J_3$ is to be understood as the spin projection along $z$. In the massive case one finds $\tanh\eta=|{\vec k}|/\sqrt{{\vec k}^2+m^2}$. 


Eq. \eqref{eq:DefHelicity} uniquely defines all states within the domain $\Theta\in[0,\pi)$ and $\Phi\in[0,2\pi)$. However, particles moving along the negative $z$ axis, i.e. those with $\Theta=\pi$, are only defined up to a phase because their azimuthal angle $\Phi$ --- appearing in the standard rotation in eq. \eqref{eq:DefHelicity} --- is not uniquely determined. We conventionally assume that $\Phi=0$ at $\Theta=\pi$, which is equivalent to
\ba\label{def-z}
|\hspace{-0.1cm}-\hspace{-0.1cm}|{\vec k}|{\vec z},h\rangle&\equiv& U(R_{\rm JW}(\pi,0)\,e^{+i\eta K_3})|{\vec k}_{\rm ref},h\rangle\\\no
&=&U(R_{\rm JW}(\pi,0))|\hspace{-0.1cm}+\hspace{-0.1cm}|{\vec k}|{\vec z},h\rangle\,,
\ea 
%However, this convention will have no practical relevance for us because by assumption the particles moving precisely on the $z$ axis are external states, and as such their phases have no physical effect. 
From these definitions we can determine the spinors and polarization vectors up to a conventional phase. The latter will be completely specified by our definitions below. 


Consider a particle of mass $m$, helicity $h$, three-momentum \eqref{3momentum} and (positive) energy $k_0=\sqrt{{\vec k}^2+m^2}$. The definition $|{\vec k}|=\sqrt{{\vec k}^2}$ will be adopted even for complex momenta. %We recall that $\Theta\in[0,\pi)$ and $\Phi\in[0,2\pi)$, with the additional point $\Theta=\pi, \Phi=0$. 
For $h=+1,-1,0$, the polarization vectors are (we use the mostly-minus metric throughout the paper)
\ba\no%\label{e_pm}
\varepsilon^+_\mu[k]=\frac{1}{\sqrt{2}}\frac{1}{|{\vec k}|(|{\vec k}|+k_z)}\left(
\begin{matrix}
0\\
|{\vec k}|(|{\vec k}|+k_z)-k_x(k_x+ik_y)\\
i|{\vec k}|(|{\vec k}|+k_z)-k_y(k_x+ik_y)\\
-(|{\vec k}|+k_z)(k_x+ik_y)
\end{matrix}
\right)
=
-\frac{e^{i\Phi}}{\sqrt{2}}\left(
\begin{matrix}
0\\
-\cos\Theta\cos\Phi+i\sin\Phi\\
-i\cos\Phi-\cos\Theta\sin\Phi\\
\sin\Theta
\end{matrix}
\right)\,,\\\no
%%%%
\varepsilon^{-}_\mu[k]=\frac{1}{\sqrt{2}}\frac{1}{|{\vec k}|(|{\vec k}|+k_z)}\left(
\begin{matrix}
0\\
-|{\vec k}|(|{\vec k}|+k_z)+k_x(k_x-ik_y)\\
i|{\vec k}|(|{\vec k}|+k_z)+k_y(k_x-ik_y)\\
(|{\vec k}|+k_z)(k_x-ik_y)
\end{matrix}
\right)
=
\frac{e^{-i\Phi}}{\sqrt{2}}\left(
\begin{matrix}
0\\
-\cos\Theta\cos\Phi-i\sin\Phi\\
i\cos\Phi-\cos\Theta\sin\Phi\\
\sin\Theta
\end{matrix}
\right)\,,
\ea
and
\begin{equation}\no%\label{e_0}
\varepsilon^{0}_\mu[k]=\frac{k_0}{m}\left(
\begin{matrix}
\frac{|{\vec k}|}{k_0}\\
-\frac{k_x}{|{\vec k}|}\\
-\frac{k_y}{|{\vec k}|}\\
-\frac{k_z}{|{\vec k}|}
\end{matrix}
\right)
=\frac{k_0}{m}\left(
\begin{matrix}
\frac{|{\vec k}|}{k_0}\\
-\sin\Theta\cos\Phi\\
-\sin\Theta\sin\Phi\\
-\cos\Theta
\end{matrix}
\right)\,.
\end{equation}
As established in \eqref{def-z}, the polarization vectors for a particle in the backward limit ${\vec k}\to(0,0,-|{\vec k}|)$ are defined taking $k_x\to0^+$ with $k_y/k_x\to0$, and of course $k_z\to-|{\vec k}|$. With this prescription the expressions of $\varepsilon^{h}_\mu[k]$ are regular and single-valued. %, despite the fact that $|{\vec k}|+k_z\to0$ in that limit, as is manifest in terms of angular variables. 


It is useful to introduce the conjugate polarizations ${\overline{\varepsilon}_\mu^h}[k]$, which appear in matrix elements with external vectors as well as the completeness relation \eqref{complE}. For arbitrary (complex) momenta they are defined as
\ba
{\overline{\varepsilon}_\mu^h}[k]\equiv(-1)^h{\varepsilon}^{-h}_\mu[k]\,.
\ea
(Note that for real momenta conjugation coincides with standard complex conjugation.) Our definitions ensure the completeness relation $\sum_h{{\varepsilon}_\mu^h}[k]{\overline{\varepsilon}_\nu^h}[k]=-\eta_{\mu\nu}+k_\mu k_\nu/m^2$ is satisfied for any complex $k^\mu$ (recall our definition $|{\vec k}|=\sqrt{{\vec k}^2}$). The $\varepsilon_\mu^h[k]$ and the completeness relation can be straightforwardly generalized to $k^2\neq m^2$ by simply replacing $m^2\to k^2$.

In the tree approximation Eqs \eqref{stdpol} and \eqref{newpol} become:
\ba
{\cal E}^\pm_M[k]&=&\left(\varepsilon^{\pm}_\mu({\vec k}),0\right)\\\no
{\cal E}^0_M[k]&=&\left(-\frac{m}{k_0+|{\vec k}|}
\left\{1,\frac{{\vec k}}{|{\vec k}|}\right\},i\right)\,.
\ea
These are the generalized polarization vectors we will use in our computation of the splitting amplitudes (see \eqref{splitGen}).

Dirac spinors for particles or anti-particles of helicity $h=\pm1/2$ are given by
\begin{equation}\label{e_uv}
u_h[k]=
\left(
\begin{matrix}
\kappa_{-h}[k]\,\chi_{h}({\vec k})\\
\kappa_{h}[k]\,\chi_{h}({\vec k})
\end{matrix}
\right),\qquad
v_h[k]=
\left(
\begin{matrix}
2h\kappa_{h}[k]\,\chi_{-h}({\vec k})\\
-2h\kappa_{-h}[k]\,\chi_{-h}({\vec k})
\end{matrix}
\right),
\end{equation}
where $\kappa_h[k]=\sqrt{k_0+2h|{\vec k}|}$ and 
\ba
&&\chi_{1/2}({\vec k})=
\frac{1}{\left[2|{\vec k}|\left(|{\vec k}|+k_z\right)\right]^{1/2}}
\left(
\begin{matrix}
|{\vec k}|+k_z\\
{k_x+ik_y}
\end{matrix}
\right)
=
\left(
\begin{matrix}
\cos\Theta/2\\
e^{i\Phi}\sin\Theta/2
\end{matrix}
\right)\,,\\
%%%%%%
&&\chi_{-1/2}({\vec k})=
\frac{1}{\left[2|{\vec k}|\left(|{\vec k}|+k_z\right)\right]^{1/2}}
\left(
\begin{matrix}
-k_x+ik_y\\
{|{\vec k}|+k_z}
\end{matrix}
\right)
=\left(
\begin{matrix}
-e^{-i\Phi}\sin\Theta/2 \\
\cos\Theta/2
\end{matrix}
\right).
\ea
Similarly to the polarizations for vector particles, the wavefunction for a $h=\pm1/2$ state with $|{\vec k}|+k_z\to0^+$ is unambiguously obtained taking the limit $k_x\to0^+$ with $k_y/k_x\to0$. 

The conjugate spinors are defined as
\ba\label{conjSpinor}
{\overline u}_h[k]&=&v_h^t[k](i\gamma^0\gamma^2)\\\no
{\overline v}_h[k]&=&u_h^t[k](i\gamma^0\gamma^2)\,,
\ea
where the $\gamma^\mu$ matrices are understood to be in the Weyl representation. The completeness relations coincide with the standard ones, namely $\sum_h u_h[k]{\overline u}_h[k]={\slashed{k}}+m$ and $\sum_h v_h[k]{\overline v}_h[k]={\slashed{k}}-m$, for arbitrary complex $k^\mu=(k^0,{\vec k})$ provided the conjugate spinors in eq. \eqref{conjSpinor} are used. Again, all our expressions can be generalized to any value of the invariant mass by taking $m^2\to k^2$.




\subsubsection*{Properties of Splitting Amplitudes}





We begin discussing the collinear splitting amplitudes $\M^{\rm split}(A\rightarrow BC)$ defined in eq. \eqref{splitGen} for the standard 3-kinematics specified in eq. \eqref{eq:kin}, where $A$ moves exactly in the positive direction of the $z$ axis. To match the notation of \eqref{3momentum} we observe that the angular variables $\Theta,\Phi$ of particles $A, B,C$ in the standard configuration read
\ba
(\Theta^{\rm std}_A,\Phi^{\rm std}_A)&=&(0,{\rm undet.})\\\no
(\Theta^{\rm std}_B,\Phi^{\rm std}_B)&=&\left({\cal O}(|{\bf k}_\bot|),\phi\right)\\\no
(\Theta^{\rm std}_C,\Phi^{\rm std}_C)&=&\left({\cal O}(|{\bf k}_\bot|),\phi\pm\pi\right)\,,
\ea
with $\Phi^{\rm std}_A$ undetermined and the $+$ or $-$ sign in $\Phi^{\rm std}_C$ depending on whether $\phi\in[0,\pi]$ or $\phi\in[\pi,2\pi]$.




Despite not being S-matrix elements, $\M^{\rm split}(A\rightarrow BC)$ transform under all symmetries as physical amplitudes. Their structure is in fact determined by dimensional analysis and angular momentum considerations. From Lorentz invariance follows that these quantities must be proportional to the soft scales $|{\bf k}_\bot|, m_{A,B,C}$, up to negligible corrections ${\cal O}(\delta_{m,\bot}^2)$. Conservation of the angular momentum further fixes the dependence on the azimuthal angle $\phi$ introduced in eq. \eqref{eq:kin} \cite{EWA_Wulzer}. Indeed, in the helicity basis defined in eq. \eqref{eq:DefHelicity} one finds that under rotations $R_{\rm JW}(0,\phi')$ around the $z$ axis the 1-particle states transform as $U(R_{\rm JW}(0,\phi'))|{\vec k},h\rangle=e^{-i\phi'h}|R_{\rm JW}(0,\phi'){\vec k},h\rangle$. Invariance under rotations then implies $\M^{\rm split}(R_{\rm JW}(0,\phi'){\bf k}_\bot,m)=e^{-i\phi'\Delta h}\M^{\rm split}({\bf k}_\bot,m)$, with $\Delta h=h_{B}+h_C-h_A$ the total change in helicity and the phase arising from the Little Group transformation of the external one-particle states. The latter condition is solved observing that the projections of ${\bf k}_\bot$ onto the eigenvectors of $J_3$, namely ${\bf k}_\bot^1\pm i{\bf k}_\bot^2=e^{\pm i \phi}|{\bf k}_\bot|\to e^{\pm i(\phi+\phi')}|{\bf k}_\bot|$, are the two linear combinations of ${\bf k}_\bot$ covariant under the action of $R_{\rm JW}(0,\phi')$. Using these considerations together with the fact that $\M^{\rm split}$ is analytic in ${\bf k}_\bot$ allows us to conclude that the splitting amplitudes must have the structure 
$$
\M^{\rm split}(A\to BC)\propto|{\bf k}_\bot|^{|\Delta h|}e^{-i\phi\Delta h}
$$ 
as shown in eq. \eqref{eq-collinear_splitting}. 

The $\M^{\rm split}$'s satisfy two additional useful relations. First, from \eqref{eq:kin} immediately follows that 
\ba\label{BCCB}
\M^{\rm split}(A_{h_A}\rightarrow C_{h_C}B_{h_B})=\left.\M^{\rm split}(A_{h_A}\rightarrow B_{h_B}C_{h_C})\right|_{\phi\to\phi+\pi,~x\to1-x,~m_B\to m_C,~m_C\to m_B}\,.
\ea
%Moreover, crossing symmetry implies (is this right?)
%\ba\label{crossing}
%\M^{\rm split}(\overline{C}_{\overline{h}_C}\rightarrow B_{h_B}\overline{A}_{\overline{h}_A})={\rm sign}(\overline{h}_A\overline{h}_C)~\M^{\rm split}(A_{-\overline{h}_A}\rightarrow B_{h_B}C_{-\overline{h}_C}).
%\ea
%Finally, 
Moreover, the accidental CP invariance of the tree-level amplitudes introduces another important constraint. Actually, rather than using parity (P) itself, we find it more convenient to consider the combined action of P and a $\pi$-rotation along the $y$-axis, i.e. P$'\equiv R_{\rm JW}(\pi,0)\,$P. The resulting operator acts on a state $|{\vec k},h,A\rangle$ describing a particle $A$ of momentum ${\vec k}$ and helicity $h$ as CP$'|{\vec k},h,A\rangle=(-1)^{j-h}\,\bar{\eta}\,|{\rm P}'{\vec k},-h,{\overline{A}}\rangle$ whereas as CP$'|{\vec k},h,\overline{A}\rangle=(-1)^{j-h}\,\bar\eta^*\,|{\rm P}'{\vec k},-h,{{A}}\rangle$ on anti-particles, where $\bar\eta$ are phases (or unitary matrices when different particle species can mix) appearing in the field transformations.~\footnote{Within our conventions the scalar $\phi(x)$, Dirac fermion $\psi(x)$, and vector $V_\mu(x)=V^a_\mu(x) T^a$ fields are assumed to transform respectively as $({\rm CP}')\phi(x)({\rm CP}')^\dagger=\bar\eta^*_\phi \phi^\dagger(x')$, $({\rm CP}')\psi(x)({\rm CP}')^\dagger=\bar\eta^*_\psi\gamma^5{\psi^\dagger}(x')$, $({\rm CP}')V_\mu(x)({\rm CP}')^\dagger=-\bar\eta^*_V (R_{\rm JW}(-\pi,0)\,{\cal P})_{\mu}^{\nu}V^\dagger_\nu(x')$, with $x'=R_{\rm JW}(\pi,0){\cal P}x$ and ${\cal P}^{\mu}_\nu={\rm diag}(1,-1,-1,-1)$.} Since ${\rm P}'{\vec k}=|{\vec k}|\left(\sin\Theta\cos\Phi,-\sin\Theta\sin\Phi,\cos\Theta\right)$ is equivalent to an inversion of the azimuthal angle, we obtain 
\ba\label{CPsplit}
\M^{\rm split}(\overline{A}_{-{h}_A}\rightarrow \overline{B}_{-h_B}\overline{C}_{-{h}_C})=\prod_{k=A,B,C}(-1)^{j_k-h_k}~~\bar\eta_{A}^*\bar\eta_{B}\bar\eta_{C}\,\left.\M^{\rm split}(A_{h_A}\rightarrow B_{h_B}C_{h_C})\right|_{\phi\to-\phi}\,.
\ea
In the SM the Higgs and the fermionic phases may be absorbed in the Yukawa couplings using chiral rotations and hyper-charge transformations so that we can set $\bar\eta_\phi=\bar\eta_\psi=1$. Moreover, real vectors have $\bar\eta_V=\pm1$. Without loss of generality, therefore, the phases $\bar\eta_{A,B,C}$ appearing in \eqref{CPsplit} can be taken to be $+1$ when the particles involved are fermions, CP-even scalars, or CP-even vectors, whereas $\bar\eta=-1$ for CP-odd scalars and vectors.



\subsubsection*{Factorization with $A$ in an arbitrary direction}


In this subsection we demonstrate that the very same $\M^{\rm split}(A\to BC)$ obtained with the standard 3-momentum given in eq. \eqref{eq:kin} can be adopted in calculations of factorized amplitudes (see eqs \eqref{fact} \eqref{fact2}) even if $A$ moves along an arbitrary direction. Let us parametrize our general kinematic configuration by rotating the standard ${\vec k}^{\rm std}_{A,B,C}$ in eq. \eqref{eq:kin} with a common matrix \ba
{\vec k}_{A,B,C}=R_{\rm JW}(\Theta_A,\Phi_A){\vec k}^{\rm std}_{A,B,C}
\ea
as in eq. \eqref{eq:kin_gen}. The action of a Jacob-Wick rotation on 1-particle states can be derived directly from the definition in eq. \eqref{eq:DefHelicity} and reads 
\ba\label{RotStates}
U(R_{\rm JW}(\Theta_A,\Phi_A))|{\vec k}^{\rm std}_A,h_A\rangle&=&|{\vec k}_A,h_A\rangle\\\no
U(R_{\rm JW}(\Theta_A,\Phi_A))|{\vec k}^{\rm std}_B,h_B\rangle&=&e^{i\Psi_B}|{\vec k}_B,h_B\rangle\\\no
U(R_{\rm JW}(\Theta_A,\Phi_A))|{\vec k}^{\rm std}_C,h_C\rangle&=&e^{i\Psi_C}|{\vec k}_C,h_C\rangle\,.
\ea
There is no phase associated to $A$ because, according to the definition in eq \eqref{eq:DefHelicity}, a rotation as in eq. \eqref{eq:kin_gen} acting on a state $A$ moving in the positive $z$ direction precisely generates a state with rotated 3-momentum. 

The same phases show up in the polarizations (for example, for a vector particle $R_{\rm JW}\varepsilon({\vec k})=e^{i\Psi}\varepsilon(R_{\rm JW}{\vec k})$) as well as in matrix elements. In particular, eq \eqref{RotStates} implies the splitting functions for the rotated states are related to those in the standard parametrization \eqref{eq:kin} by
\ba\label{RotPhase}
\M^{\rm split}(A_{{\vec k}_A}\rightarrow B_{{\vec k}_B}C_{{\vec k}_C})&=&e^{i(\Psi_B+\Psi_C)}\M^{\rm split}(A_{{\vec k}^{\rm std}_A}\rightarrow B_{{\vec k}^{\rm std}_B}C_{{\vec k}^{\rm std}_C})\\\no
&\equiv&e^{i(\Psi_B+\Psi_C)}\left.\M^{\rm split}\right|_{{\vec k}_A={\vec k}_A^{\rm std}}\,.
\ea
Obviously not all phases in eq. \eqref{RotPhase} are physical. This is because in a splitting process two of the states involved are necessarily on-shell. Hence, phases associated to the latter eventually disappear from any observable and can be ignored. Only the phase of the virtual state can potentially be relevant in the calculation of the factorized amplitude. In the case of splitting in the final state $A^*\to BC$ the only relevant phase  would thus be the one associated to $A$, but this vanishes by construction (see eq. \eqref{RotPhase}). As a result, in the analysis of an arbitrary (single and multiple) final state splitting we can safely use in eq. \eqref{fact2} the splitting functions $\M^{\rm split}(A\rightarrow BC)$ calculated with the standard 3-kinematics specified in eq. \eqref{eq:kin}. 




Consider next a splitting $A\to BC^*$ of the initial state. Here $B$ is on-shell by convention, and so $e^{i\Psi_B}$ is again unphysical. The case of a single splitting in the initial state, when $A$ moves exactly along the positive $z$ axis, has been studied before and by definition $e^{i(\Psi_B+\Psi_C)}=1$ in that case. If multiple splittings occur, however, some of the initial state particles are slightly tilted from the $z$ axis. These are thus associated to initial state splittings in which the corresponding $A$ state is rotated by a small $\Theta_A\ll\pi$. An explicit computation shows that $\Psi_{C}={\cal O}(\delta_\bot)$ in such a situation.~\footnote{This is strictly true only for $\pi-\Theta_A\gg{\cal O}(\delta_\bot)$. The same calculation shows that $\Psi_{B}={\cal O}(\delta_\bot)$ as well, though this is not relevant in our discussion.} This guarantees that, when considering multiple splittings from an initial state moving along the positive $z$ axis, the phase in eq. \eqref{RotPhase} at most affects the subleading term in eq. \eqref{fact}.

Because of the ambiguity in the definition of backward-moving particles (see the discussion around eq. \eqref{def-z}), the situation is a bit more involved when the initial state splitting takes place from an original particle $A$ moving in the direction of the negative $z$ axis. The phase $e^{i\Psi_C}$ in eq. \eqref{RotPhase} in fact becomes of order unity when $\pi-\Theta_A\lesssim{\cal O}(\delta_\bot)$ and superficially might invalidate our claim. Fortunately, though, the ${\cal O}(1)$ contribution to $\Psi_C$ gets partly compensated by an analogous and opposite phase showing up in the hard process when taking the collinear limit, leaving in the end a negligible correction of ${\cal O}(\delta_\bot)$ to the factorized amplitude, similarly to the previous case. To see this recall that in eq. \eqref{fact} the splitting amplitude is multiplied by an S-matrix element $i{\cal M}^{\rm hard}(C X\to Y)$ %\equiv\langle Y|S\left(|X\rangle\otimes |{{\vec k}'_C},h_C\rangle\right)$, 
calculated for an on-shell $C$ moving along an arbitrary direction ${\vec k}_C=R_{\rm JW}(\Theta_A,\Phi_A){\vec k}^{\rm std}_C$ identified by the new direction of $A$ (i.e. by $\Theta_A, \Phi_A$) and the standard variables $\Phi^{\rm std}_B\equiv\phi, \Theta^{\rm std}_B={\cal O}(\delta_\bot)$. A trivial use of eq. \eqref{RotStates} shows that 
\ba\label{hardNew}
{\cal M}^{\rm hard}(C_{{\vec k}_C} X\to Y)=e^{-i\Psi_C}{\cal M}^{\rm hard}(C_{{\vec k}_C}^{\Psi} X\to Y)\,,
\ea
where ${\cal M}^{\rm hard}(C^{\Psi} X\to Y)$ is the analogous hard matrix element for a non-standard state $|{{\vec k}_C},h_C\rangle^{\Psi}\equiv e^{i\Psi_C}|{\vec k}_C,h_C\rangle$ %=U(R_{\rm JW}(\Theta_A,\Phi_A))|{{\vec k}^{\rm std}_C},h_C\rangle$ 
that includes the phase in \eqref{RotStates}. The advantage of this simple manipulation is twofold. By definition of $|{{\vec k}_C},h_C\rangle^{\Psi}$, the phase $e^{i\Psi_C}$ completely disappears from the factorized amplitude when the hard amplitude in eq. \eqref{hardNew} is multiplied by \eqref{RotPhase}. Furthermore, it turns out the non-standard state $|{{\vec k}_C},h_C\rangle^{\Psi}$ involved in the hard process smoothly approaches a conventional Jacob-Wick state in the collinear limit, defined such that ${\vec k}_{C}$ becomes a vector ${\vec k}_{C, {\rm coll}}\equiv {\vec k}_A\cdot|{\vec k}_C|/|{\vec k}_A|$ parallel to ${\vec k}_{A}$, or equivalently by taking $\Theta^{\rm std}_B={\cal O}(\delta_\bot)\to0$. Indeed, using eq. \eqref{RotStates}, and thanks to the fact that $R_{\rm JW}(\Theta^{\rm std}_B,\Phi^{\rm std}_B)\to1$ smoothly, we have
\ba\label{collCdef}
\lim_{\delta_\bot\to0}|{{\vec k}_C},h_C\rangle^{\Psi}%&\equiv&\lim_{\delta_\bot\to0}U(R_{\rm JW}(\Theta_A,\Phi_A))|{{\vec k}_C},h_C\rangle\\\no
&\equiv&\lim_{\delta_\bot\to0}U(R_{\rm JW}(\Theta_A,\Phi_A)\cdot R_{\rm JW}(\Theta^{\rm std}_B,\Phi^{\rm std}_B))|\hspace{-0.1cm}+\hspace{-0.1cm}|{\vec k}_C|{\vec z},h_C\rangle
\\\no
&=&U(R_{\rm JW}(\Theta_A,\Phi_A))|\hspace{-0.1cm}+\hspace{-0.1cm}|{\vec k}_C|{\vec z},h_C\rangle\\\no
&\equiv&|{\vec k}_{C, {\rm coll}},h_C\rangle\,,
\ea
with no phase whatsoever irrespective of the value of $\Theta_A$. The result in eq. \eqref{collCdef} is to be contrasted with the collinear limit of the Jacob-Wick state $|{\vec k}_C,h_C\rangle$ in eq. \eqref{RotStates}, which reads $e^{-i\Psi_C^0}|{\vec k}_{C, {\rm coll}},h_C\rangle$, where $\Psi_C^0=\lim_{\delta_\bot\to0}\Psi_C$ is in general non-vanishing due to the ambiguity we encountered in the definition of 1-particle states with $\Theta\to\pi$.~\footnote{For example, in the case $\Theta_A=\pi, \Phi_A=0$ in which $A$ exactly moves in the negative $z$ direction one has $|{\vec k}_C,h_C\rangle%=U(R_{\rm JW}(\pi-\Theta_C^{\rm std},2\pi-\phi))||{\vec k}_C|{\vec z},h_C\rangle
\to U(R_{\rm JW}(\pi,2\pi-\phi))|\hspace{-0.1cm}+\hspace{-0.1cm}|{\vec k}_C|{\vec z},h_C\rangle%=e^{-2i\phi h_C}U(R_{\rm JW}(\pi,0)||{\vec k}_C|{\vec z},h_C\rangle
=e^{-2i\phi h_C}|\hspace{-0.1cm}-\hspace{-0.1cm}|{\vec k}_C|{\vec z},h_C\rangle$, or equivalently $\Psi_C^0=2\phi h_C={\cal O}(1)$. %The left over phase is exactly the same that renders multi-valued the polarization vectors evaluated at $\Theta_C\to\pi$.
}
Finally, combining eqs. \eqref{RotPhase}, \eqref{hardNew}, and \eqref{collCdef} we conclude that the factorized amplitude in eq. \eqref{fact} becomes
\ba\no
i\M^{({\rm fact})}(A_{{\vec k}_A}X\to B_{{\vec k}_B}Y)&=&\sum_Ci{\cal M}^{\rm hard}(C_{{\vec k}_C} X\to Y)\frac{i}{Q^2}i\M^{\rm split}(A_{{\vec k}_A}\rightarrow B_{{\vec k}_B}C^*_{{\vec k}_C})\\\no
&=&\left.\sum_Ci{\cal M}^{\rm hard}(C_{{\vec k}_{C, {\rm coll}}} X\to Y)\frac{i}{Q^2}i\M^{\rm split}\right|_{{\vec k}_A={\vec k}_A^{\rm std}}e^{i\Psi_B}\left[1+{\cal O}(\delta_\bot)\right]\,.
\ea
This expression is formally the same as the one given in eq. \eqref{fact} apart from an unphysical phase and the replacements $k^\mu_C\to k^\mu_{C,{\rm coll}}$ and $\left.\M^{\rm split}(A_{{\vec k}_A}\rightarrow B_{{\vec k}_B}C^*_{{\vec k}_C})\to\M^{\rm split}\right|_{{\vec k}_A={\vec k}_A^{\rm std}}$. 

We have thus established that, without loss of generality, the factorized amplitudes with $A$ in an arbitrary direction can be calculated using the splitting functions derived with the standard 3-kinematics in eq. \eqref{eq:kin}.

 
% (single or multiple)












%Because of the ambiguity in the definition of backward particles we have seen around \eqref{def-z}, the situation is a bit more involved when the initial state splitting takes place from an original particle $A$ moving along the negative $z$ axis. The relevant phase $e^{i\Psi_C}$ in eq. \eqref{RotPhase} in fact becomes of order unity when $\pi-\Theta_A\lesssim{\cal O}(\delta_\bot)$. Consider for example the splitting from an initial $A$ exactly in the negative $z$ axis. Taking $\Theta_A=\pi, \Phi_A=0$ we obtain
%\ba
%e^{i(\Psi_B+\Psi_C)}=(-1)^{2j_B}e^{-2i\phi h_B}e^{-2i\phi h_C}\,,
%\ea
%where the left over phase $e^{-2i\phi h_C}$ is unsuppressed. Not surprisingly, however, the latter is exactly compensated by a large phase that survives in the collinear limit of the hard amplitude, when ${\vec k}_{C'}$ is taken parallel to ${\vec k}_{A'}$. 









\subsection{Splitting Amplitudes for a General Gauge Theory}
\label{app:splittingList}


We now present the Feynman rules relevant for the evaluation of the splitting functions in the tree approximation, namely those associated to 3-particle vertices. We parametrize the couplings in terms of generic functions $C_{ABC}$ so that our results can be straightforwardly applied to general renormalizable gauge theories. An explicit expression for $C_{ABC}$ is presented in the case of the SM. We subsequently collect all the independent splitting amplitudes arising from the Feynman rules. The unlisted amplitudes can be obtained from \eqref{BCCB} and \eqref{CPsplit}. 

\newpage 

\subsubsection*{Relevant Feynman Rules}


\begin{itemize} 
\item Fermionic Vertices
\end{itemize} 


The interaction vertices between two fermions $f^a, f^b$ of masses $m_{a,b}$ and a vector boson $V$ or a scalar $h$ are defined below in terms of general couplings $C_{L,R}$, $y_f$, and $P_{L}=({1-\gamma_5})/{2}$, $P_{R}=({1+\gamma_5})/{2}$ denoting the chirality projectors. 


In the SM the Yukawa coupling $y_f$ is diagonal in fermion flavor and related to the fermion mass $m_f=m_a=m_b$ through the Higgs VEV as $y=\sqrt{2} m_f/v$, whereas the parameters $C_{L,R}$ are collected in this table

%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{center}
\begin{tabular}{c|cccc} 
\rule{0pt}{1.2em}%
$V$ & $W^-~(f^a=d, f^b=u)$ &  $Z~(f^a=f^b)$ &  $\gamma~(f^a=f^b)$ & $G~(f^a=f^b)$  \\
\hline
$C_L$ & $\frac{gV_{ud}}{\sqrt{2}}$ &  $\frac{g}{c_{\rm w}}(T^3-s_{\rm w}^2q_f)$ &  $eq_f$ & $g_st^\alpha_{i_bi_a}$  \\
$C_R$ & $0$ &  $\frac{g}{c_{\rm w}}(-s_{\rm w}^2q_f)$ &  $eq_f$ & $g_st^\alpha_{i_bi_a}$  
\end{tabular}
\end{center}
%\caption{\small Vector couplings of the SM fermions. Here $V_{ud}$ is an element of the CKM matrix, $T^A$ are the weak SU$(2)$ and $t^\alpha$ the color SU$(3)$ generators in the fundamental representation, $e=g s_{\rm w}$ ($g_s$) is the QED (QCD) coupling and finally $q_f$ is the electric charge.
%\label{CLCR}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%






\vspace{-10pt}

\noindent
Here $V_{ud}$ is an element of the CKM matrix, $T^A$ are the weak SU$(2)$ and $t^\alpha$ the color SU$(3)$ generators in the fundamental representation, $e=g s_{\rm w}$ ($g_s$) is the QED (QCD) coupling and finally $q_f$ is the electric charge.

The Feynman rule for the coupling between two fermions and a Goldstone boson $\pi$, when present, may be derived from the $f^af^bV$ vertex using the tree-level version of the generalized Ward identity in eq. \eqref{genWardgen}, $ik^\mu\mA\left\{V_\mu[k]\right\}=-m_V\mA\left\{\pi[k]\right\}$, and the Dirac equation. Note that $m_V$ is the mass of the vector associated to the Goldstone boson. %For the SM photon ($\gamma$) and gluon ($G$) we have $C_L=C_R$, $m_a=m_b=m_f$, and consistently there is no coupling to Goldstones. 



\ba\no%\label{ffV}
~~~~~~~~~~~~~~~~~~~~
\includegraphics[scale=1.1,left]{figs/2f1V_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2f1pi_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2f1h_vertex.pdf}
\ea







\newpage

\begin{itemize} 
\item Bosonic Scalar Vertices
\end{itemize} 



We now move to purely bosonic vertices involving at least a scalar particle. The Feynman rule for the cubic scalar coupling is defined as $-i6\lambda v$. In the SM $\lambda$ is the quartic Higgs coupling and $v$ its VEV. In the case of general scalar theories one just replaces $6\lambda v$ with the appropriate trilinear. Vertices with two scalars and one Goldstone are forbidden. On the other hand, vertices of the type $h\pi^a\pi^b$ are related to the $hV^aV^b$ vertex via \eqref{genWardgen}.


Renormalizable $hV^a V^b$ vertices, with a scalar boson and two massive vectors, are parametrized in general in terms of a dimensionful coupling $C\sqrt{m_{V_a}m_{V_b}}$. In the Standard model this is given by:

\vspace{-5pt}

%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{center}
\begin{tabular}{c|cccc} 
\rule{0pt}{1.2em}%
$V^a V^b$ & $W^-W^+$ &  $ZZ$ & $\gamma\gamma$ & $GG$\\
\hline
$C\sqrt{m_{a}m_{b}}$ & $gm_W$ &  $\frac{g}{c_{\rm w}}m_Z$ & $0$ & $0$
\end{tabular}
\end{center}\label{HVV}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%


\vspace{-15pt}

\noindent
Similarly to the fermionic couplings to Goldstone bosons and $h\pi^a{\pi}^b$, the vertex $h\pi^a{V}^b$ written below can be shown to be related to $hV^a V^b$ via the generalized Ward identity. 

{A vertex with two scalars and a transverse vector should also be included in general, though absent in the SM. Without loss of generality we assume the very same Feynman rule as $h\pi^a{V}^b$, and the associated splitting amplitudes are shown at the very end of our list with $\pi\to h'$.}




\ba\no
~~~~~~~~~~~~~~~~~~~~
\includegraphics[scale=1.1, left]{figs/3h_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2V1h_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/Vpih_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2pi1h_vertex.pdf}
\ea

\vspace{9pt}





\newpage

\begin{itemize} 
\item Vector and Goldstone Vertices
\end{itemize} 


Finally, we present the Feynman rules for three vector and Goldstone bosons. The most general (renormalizable) vertex involving three vectors depends on a coupling $C_{abc}$, which is fully antisymmetric in the three indices $a,b,c$. In the SM

%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{center}
\begin{tabular}{c|ccc} 
\rule{0pt}{1.2em}%
$V^aV^bV^c$ & $W^-W^+\gamma$ &  $W^-W^+Z$ & $G^\alpha G^\beta G^\gamma$\\
\hline
$C_{abc}$ & $e$ &  $g c_{\rm w}$ & $-ig_sf_{\alpha\beta\gamma}$ 
\end{tabular}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%


\vspace{-10pt}

\noindent
with $f_{\alpha\beta\gamma}$ denoting the SU$(3)$ structure constants. The corresponding vertices with one or two Goldstone bosons, when present, are related to the three-vector vertex via the generalized Ward identity in eq. \eqref{genWardgen}. No three-Goldstone vertex can arise from spontaneous breaking. This can also be explicitly confirmed using eq. \eqref{genWardgen}.


\ba\no
~~~~~~~
\includegraphics[scale=1.1,left]{figs/3V_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2V1pi_vertex.pdf}
\\\no\\\no
\includegraphics[scale=1.1,left]{figs/2pi1V_vertex.pdf}
\ea






\newpage

%\pagebreak
%%%%%%%%%%%
\subsubsection*{Splitting Amplitudes}
\begin{itemize}
\item Fermions and Vectors
\end{itemize}
%%%%%%%%%%%





%\vspace{0.1cm}

\begin{table}[h]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_ffV.pdf}
\vspace{0.2cm}

%\begin{tabular}{ c||c|c|c|c }
%$\rightarrow$ & $f^b_{-1/2}+V_1$ & $f^b_{-1/2}+V_{-1}$ & 
%$f^b_{1/2}+V_1$ & $f^b_{1/2}+V_{-1}$
% \\ \hline \hline
%$f^a_{-1/2}$ & $\sqrt{2}C_L \frac{\sqrt{1- x} }{x}|{\bf k}_{\bot}| e^{-i \phi }$ & 
%$-\sqrt{2}C_L|{\bf k}_{\bot}|\frac{   e^{i \phi }}{x\sqrt{1- x} }$ 
%& $0$
%& $\sqrt{2} C_L\frac{ m_b}{\sqrt{1-x}}-\sqrt{2}C_R m_a \sqrt{1-x}$
% \\ \hline
%$f^a_{1/2}$ & $\sqrt{2} C_R\frac{m_b }{\sqrt{1-x}}-\sqrt{2}C_L m_a \sqrt{1-x} $ 
%& $0$ 
%& $\sqrt{2}C_R|{\bf k}_{\bot}|\frac{  e^{-i \phi } }{x\sqrt{1-x} }$
%& $-\sqrt{2}C_R\frac{ \sqrt{1- x}}{x} |{\bf k}_{\bot}| e^{i \phi }$
%\end{tabular}
\begin{tabular}{ c||c|c }
$\rightarrow$ & $f^b_{-1/2}+V_1$ & $f^b_{-1/2}+V_{-1}$ 
 \\ \hline \hline
$f^a_{-1/2}$ & $\sqrt{2}C_L \frac{\sqrt{1- x} }{x}|{\bf k}_{\bot}| e^{-i \phi }$ & 
$-\sqrt{2}C_L|{\bf k}_{\bot}|\frac{   e^{i \phi }}{x\sqrt{1- x} }\hphantom{-}$ 
 \\ \hline
$f^a_{1/2}$ & $\sqrt{2} C_R\frac{m_b }{\sqrt{1-x}}-\sqrt{2}C_L m_a \sqrt{1-x} $ 
& $0$ 
\end{tabular}
\vspace*{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ & $f^b_{1/2}+V_1$ & $f^b_{1/2}+V_{-1}$
 \\ \hline \hline
$f^a_{-1/2}$ 
& $0$
& $\sqrt{2} C_L\frac{ m_b}{\sqrt{1-x}}-\sqrt{2}C_R m_a \sqrt{1-x}$
 \\ \hline
$f^a_{1/2}$ 
& $\hphantom{-}\sqrt{2}C_R|{\bf k}_{\bot}|\frac{  e^{-i \phi } }{x\sqrt{1-x} }\hphantom{-}$
& $-\sqrt{2}C_R\frac{ \sqrt{1- x}}{x} |{\bf k}_{\bot}| e^{i \phi }$
\end{tabular}
%\caption{Amplitudes for a fermion splitting into another fermion and a transverse vector.}
\end{table}






\begin{table}[h]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_Vff.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c|c }
$\rightarrow$ 
& $\bar{f}^b_{-1/2}+f^a_{-1/2}$ 
& $\bar{f}^b_{1/2}+f^a_{-1/2}$
& $\bar{f}^b_{-1/2}+f^a_{1/2}$
& $\bar{f}^b_{1/2}+f^a_{1/2}$
 \\ \hline \hline
$V_{1}$ & $0$ 
& $-\sqrt{2} C_L \sqrt{\frac{1-x}{x}}|{\bf k}_{\bot}| e^{i \phi }$ 
& $\sqrt{2}C_R  \sqrt{\frac{x}{1-x}} |{\bf k}_{\bot}| e^{i \phi } $
& $-\sqrt{2}\left(C_L m_a\sqrt{\frac{ 1-x }{x}}
+C_R m_b \sqrt{\frac{x}{1-x}}\right)$ 
% \\ \hline
%$V_{-1}$ 
%& $-\sqrt{2}\left(C_L\frac{ m_2 \sqrt{x} }{\sqrt{1-x }}
%+C_R m_1 \sqrt{\frac{1-x}{x}}\right)$ 
%& $-\sqrt{2}C_L\sqrt{\frac{  x }{1-x}}|{\bf k}_{\bot}| e^{-i \phi }$ 
%& $\sqrt{2} C_R \sqrt{\frac{1-x}{x}} |{\bf k}_{\bot}| e^{-i \phi } $
%&
\end{tabular}
%\caption{Amplitudes for a transverse vector splitting into a fermion-antifermion pair.}
\end{table}



%\clearpage
%\newpage
%\pagebreak
%%%%%%%%%%%%%%%%
%\subsubsection*{Splitting: Fermions and $V_{0}$}
%%%%%%%%%%%%%%%%







\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_ffV0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ & $f^b_{-1/2}+V_0$ & $f^b_{1/2}+V_{0}$ 
 \\ \hline \hline
$f^a_{-1/2}$ 
& $C_L\left[\frac{m_a^2 (1-x) -m_b^2 }{m_V \sqrt{1-x}}
-\frac{2 m_V \sqrt{1-x}}{x}\right]+C_R\frac{m_a m_b x }{m_V \sqrt{1-x}}$ 
& $\left(\frac{m_a}{m_V}C_R-\frac{m_b}{m_V}C_L\right)
|{\bf k}_{\bot}|\frac{  e^{-i \phi }}{ \sqrt{1-x}}$
   \\ \hline
$f^a_{1/2}$ & $\left(\frac{m_b}{m_V} C_R-\frac{m_a}{m_V} C_L\right)
|{\bf k}_{\bot}|\frac{ e^{i \phi } }{\sqrt{1-x}}$
 & $C_R\left[\frac{m_a^2 (1-x) -m_b^2 }{m_V \sqrt{1-x}}
 -\frac{2 m_V \sqrt{1-x}}{x}\right]+C_L\frac{m_a m_b x }{m_V \sqrt{1-x}}$
\end{tabular}
%\caption{Amplitudes for a fermion splitting into another fermion and a longitudinal vector.}
\end{table}





\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_V0ff.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ 
& $\bar{f}^b_{-1/2}+f^a_{-1/2}$ 
& $\bar{f}^b_{1/2}+f^a_{-1/2}$
 \\ \hline \hline
$V_{0}$ 
& $\left(\frac{m_a }{m_V}C_R-\frac{m_b }{m_V}C_L\right) 
|{\bf k}_{\bot}|\frac{ e^{i \phi }}{\sqrt{x(1-x)}}$ 
& $C_L\frac{(1-x)m_a^2+x m_b^2 -2 m_V^2 x (1-x)}{m_V \sqrt{x (1-x)}}-C_R\frac{m_a m_b}{m_V \sqrt{x (1-x)}}$ 
\end{tabular}
%\caption{Amplitudes for a longitudinal vector splitting into a fermion-antifermion pair.}
\end{table}



\clearpage
%\newpage
%\pagebreak
%%%%%%%%%%%%%%%%
\begin{itemize}
\item Fermions and Scalars
\end{itemize}
%%%%%%%%%%%%%%%%




\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_ffh.pdf}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\includegraphics[scale=0.9]{figs/Split_hff.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ & $f^b_{-1/2}+h$ & $f^b_{1/2}+h$ 
 \\ \hline \hline
$f^a_{-1/2}$ 
& $-\frac{y_f}{\sqrt{2}}\frac{ m_b+m_a(1-x)}{\sqrt{1-x}}$ 
& $-\frac{y_f}{\sqrt{2}}|{\bf k}_{\bot}|\frac{  e^{-i \phi }}{\sqrt{1-x}}$
   \\ \hline
$f^a_{1/2}$ & $\frac{y_f}{\sqrt{2}}|{\bf k}_{\bot}| \frac{ e^{i \phi }}{\sqrt{1-x}}$
 & $-\frac{y_f}{\sqrt{2}}\frac{m_b+m_a (1-x)}{\sqrt{1-x}}$
\end{tabular}
%%%%%%%%%%%%%%
~~~~~~~
%%%%%%%%%%%%%%%
\begin{tabular}{ c||c|c }
$\rightarrow$ 
& $\bar{f}^a_{-1/2}+f^b_{-1/2}$ 
& $\bar{f}^a_{1/2}+f^b_{-1/2}$
 \\ \hline \hline
$h$ 
& $-\frac{y_f}{\sqrt{2}}|{\bf k}_{\bot}|\frac{  e^{i \phi }}{\sqrt{x(1-x)}}$ 
& $-\frac{y_f}{\sqrt{2}}\frac{m_b (1-x)-m_ax }{\sqrt{x(1-x)}}$ 
\end{tabular}
\end{table}

%\begin{table}[h]
%\renewcommand*{\arraystretch}{1.4}
%\centering
%\includegraphics[scale=0.9]{figs/Split_hff.pdf}
%\vspace{0.3cm}

%\begin{tabular}{ c||c|c }
%$\rightarrow$ 
%& $\bar{f}_{-1/2}+f_{-1/2}$ 
%& $\bar{f}_{1/2}+f_{-1/2}$
% \\ \hline \hline
%$h$ 
%& $-\frac{y_f}{\sqrt{2}}|{\bf k}_{\bot}|\frac{  e^{i \phi }}{\sqrt{x(1-x)}}$ 
%& $-\frac{y_f}{\sqrt{2}}m_f\frac{  (1-2 x) }{\sqrt{x(1-x)}}$ 
%\end{tabular}
%%\caption{Amplitudes for a Higgs splitting into a fermion-antifermion pair.}
%\end{table}





%\newpage
%\pagebreak
%%%%%%%%%%%
\begin{itemize}
\item Triple Scalar and Scalar-Vector Splittings
\end{itemize}
%%%%%%%%%%%



\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_hhh.pdf}\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_hV0V0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ 
& $h+h$ 
& ${V}^b_{0}+V^a_0$
 \\ \hline \hline
$h$ 
& $-\frac{3}{2}g\frac{m_h^2}{m_W}$ 
& $\frac{C}{2}\left[\frac{m_h^2}{\sqrt{m_am_b}}-m_a\sqrt{\frac{m_a}{m_b}}\frac{2-x}{x}-m_b\sqrt{\frac{m_b}{m_a}}\frac{1+x}{1-x}\right]$ 
\end{tabular}
%\caption{Amplitudes for a Higgs splitting into two Higgs or two longitudinal vectors.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_hVV.pdf}
\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_hV0V.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c }
$\rightarrow$ 
& ${V}^b_1+V^a_1$ 
& ${V}^b_{1}+V^a_{-1}$
& ${V}^b_{1}+V^a_{0}$
 \\ \hline \hline
$h$ 
& $0$ 
& $C \sqrt{m_am_b}$ 
& $-C\sqrt{\frac{m_b}{m_a}}|{\bf k}_{\bot}|\frac{e^{-i \phi }}{\sqrt{2} (1-x)}$
\end{tabular}
%\caption{Amplitudes for a Higgs splitting into a transverse vector and a transverse or longitudinal vector.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_VhV.pdf}
\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_VhV0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c }
$\rightarrow$ 
& $h+V^b_1$ 
& $h+V^b_{-1}$
& $h+V^b_{0}$
 \\ \hline \hline
$V^a_1$ 
& $-C \sqrt{m_am_b}$ 
& $0$
& $-C\sqrt{\frac{m_a}{m_b}}|{\bf k}_{\bot}|\frac{ e^{i \phi }}{\sqrt{2}}$ 
\end{tabular}
%\caption{Amplitudes for a transverse vector splitting into a Higgs and a transverse or longitudinal vector.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_V0hV.pdf}
\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_V0hV0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c }
$\rightarrow$ 
& $h+V^b_1$ 
& $h+V^b_{-1}$
& $h+V^b_{0}$
 \\ \hline \hline
$V^a_0$ 
& $C\sqrt{\frac{m_b}{m_a}}|{\bf k}_{\bot}| \frac{e^{-i \phi }}{\sqrt{2} x}$ 
& $-C\sqrt{\frac{m_b}{m_a}}|{\bf k}_{\bot}| \frac{e^{i \phi }}{\sqrt{2} x}$ 
& $\frac{C}{2}\left[-\frac{m_h^2}{\sqrt{m_am_b}}+m_a\sqrt{\frac{m_a}{m_b}}(1-2x)-m_b\sqrt{\frac{m_b}{m_a}}\frac{2-x}{x}\right]$
\end{tabular}
%\caption{Amplitudes for a longitudinal vector splitting into a Higgs and a transverse or longitudinal vector.}
\end{table}


\newpage
%\pagebreak
%%%%%%%%%%%
\begin{itemize}
\item Triple Vector Splittings
\end{itemize}
%%%%%%%%%%%



\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_VVV.pdf}
\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_V0VV.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c|c }
$\rightarrow$ 
& $V^b_1+V_1^c$ 
& $V^b_1+V_{-1}^c$
& $V^b_{-1}+V_{1}^c$
& $V^b_{-1}+V_{-1}^c$
 \\ \hline \hline
$V_1^a$ 
& $-\sqrt{2}C_{abc} |{\bf k}_{\bot}|\frac{ e^{-i \phi }}{x(1-x)}$ 
& $\sqrt{2}C_{abc}\frac{(1-x)}{x}|{\bf k}_{\bot}|  e^{i \phi }$ 
& $\sqrt{2}C_{abc}\frac{x }{1-x}|{\bf k}_{\bot}| e^{i \phi }$
& $0$
\\ \hline 
$V_0^a$ 
& $0$ 
& $C_{abc}\frac{m_c^3-m_b^2+(1-2x)m_a^2}{m_1}$ 
& $C_{abc}\frac{m_c^3-m_b^2+(1-2x)m_a^2}{m_1}$
& $0$
\end{tabular}
%\caption{Amplitudes for a transverse or longitudinal vector splitting into two transverse vectors.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_VVV0.pdf}
\hspace{1cm}
\includegraphics[scale=0.9]{figs/Split_VV0V0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c|c }
$\rightarrow$ 
& $V^b_1+V_0^c$ 
& $V^b_{-1}+V_{0}^c$
& $V^b_{0}+V_{0}^c$
 \\ \hline \hline
$V_1^a$ 
& $C_{abc}\left[\frac{ m_b^2-m_a^2}{m_c}+m_c\frac{ (2-x)}{x}\right]$ 
& $0$ 
& $-\frac{C_{abc}}{\sqrt{2}}\frac{  m_b^2+m_c^2-m_a^2}{m_bm_c} 
|{\bf k}_{\bot}| e^{i \phi }$
\end{tabular}
%\caption{Amplitudes for a transverse vector splitting into a longitudinal vector and a longitudinal or transverse vector.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_V0VV0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c|c }
$\rightarrow$ 
& $V^b_1+V_0^c$ 
& $V^b_{-1}+V_0^c$ 
 \\ \hline \hline
$V_0^a$ 
& $-\frac{C_{abc}}{\sqrt{2}}\frac{ m_a^1+m_c^2-m_b^2}{m_a m_c (1-x)}
|{\bf k}_{\bot}| e^{-i \phi }$ 
& $\frac{C_{abc}}{\sqrt{2}}\frac{ m_a^1+m_c^2-m_b^2}{m_a m_c(1-x)}
|{\bf k}_{\bot}| e^{i \phi }$
\end{tabular}
%\caption{Amplitudes for a longitudinal vector splitting into a longitudinal vector and a transverse vector.}
\end{table}

\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_V0V0V0.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c }
$\rightarrow$ 
& $V^b_{0}+V_{0}^c$
 \\ \hline \hline
$V_0^a$ 
& $\frac{C_{abc}}{2 m_a m_b m_c}
\left[m_a^2(m_b^2+m_c^2-m_a^2)(1-2x)
-m_b^2(m_a^2+m_c^2-m_b^2)\frac{1+x}{1-x}
+m_c^2(m_a^2+m_b^2-m_c^2)\frac{2-x}{x}
\right]$
\end{tabular}
%\caption{Amplitude for a longitudinal vector splitting into two longitudinal vectors.}
\end{table}






%%%%%%%%%%%%%%%%
\begin{itemize}
\item Scalars and Transverse Vector (absent in the SM)
\end{itemize}
%%%%%%%%%%%%%%%%




\begin{table}[h!]
\renewcommand*{\arraystretch}{1.4}
\centering
\includegraphics[scale=0.9]{figs/Split_hhV.pdf}~~~~~~~~~~~~~~~~~~~~~~~\includegraphics[scale=0.9]{figs/Split_Vhh.pdf}
\vspace{0.2cm}

\begin{tabular}{ c||c }
$\rightarrow$ & $h+V_{+1}$  
 \\ \hline \hline
$h'$ 
& $\frac{C}{\sqrt{2}}|{\bf k}_{\bot}|\frac{  e^{-i \phi }}{x}$
\end{tabular}
%%%%%%%%%%%%%%
~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%%%%%%%%%%%%%%
\begin{tabular}{ c||c }
$\rightarrow$ 
& $h'+h$ 
 \\ \hline \hline
$V_{+1}$ 
& $-\frac{C}{\sqrt{2}}|{\bf k}_{\bot}|  e^{i \phi }$
\end{tabular}
\end{table}






\clearpage

\bibliography{Biblio}



\bibliographystyle{JHEP.bst}
	
	
\newpage

\end{document}


